Universal equivalence of general linear groups over local rings with 1/2

In this study, it is proven that the universal equivalence of general linear groups (admitting the inverse-transpose automorphism) of orders greater than $2$, over local, not necessarily commutative rings with $1/2$, is equivalent to the coincidence of the orders of the groups and the universal equivalence of the corresponding rings.

==> header.tex <==
\ProvidesFile{header.tex}[header]

\begin{center}
{\bf Universal equivalence of general linear groups\\over local rings with $1/2$}

\smallskip
Galina Kaleeva

galinakaleeva@yandex.ru
\end{center}

{\bf Key words:} universal equivalence, general linear group, non-commutative local rings.

{\bf Abstract.}
In this study, it is proven that the universal equivalence of general linear groups (admitting the inverse-transpose automorphism) of orders greater than $2$, over local, not necessarily commutative rings with $1/2$, is equivalent to the coincidence of the orders of the groups and the universal equivalence of the corresponding rings.

==> section_1_intro.tex <==
\ProvidesFile{section_1_intro.tex}[section 1 intro]

\section{Introduction}

This work is devoted to the study of the universal equivalence of linear groups over local rings and includes a generalization of the result from the work \cite{Kaleeva} to non-commutative rings in the case of general linear groups. The author expresses gratitude to their academic advisor, Prof. Elena Igorevna Bunina, for her invaluable contribution to the research and her help and support at all stages of solving the scientific problem. The author also holds dear the memory of  Prof. Alexander Vasilievich Mikhalev and is sincerely thankful for our enriching discussions and his insightful contributions to the formulation of this research problem.
